SoK: Anti-Facial Recognition Technology

The rapid adoption of facial recognition (FR) technology by both government and commercial entities in recent years has raised concerns about civil liberties and privacy. In response, a broad suite of so-called "anti-facial recognition" (AFR) tools has been developed to help users avoid unwanted facial recognition. The set of AFR tools proposed in the last few years is wide-ranging and rapidly evolving, necessitating a step back to consider the broader design space of AFR systems and long-term challenges. This paper aims to fill that gap and provides the first comprehensive analysis of the AFR research landscape. Using the operational stages of FR systems as a starting point, we create a systematic framework for analyzing the benefits and tradeoffs of different AFR approaches. We then consider both technical and social challenges facing AFR tools and propose directions for future research in this field.

==> Makefile <==
LATEX=latex
BIBTEX=bibtex
BIBFILE=references.bib
PAPER=facesok

TEXFILES = facesok.tex \
	intro.tex \
	back.tex \
	dataflow.tex \
	stages.tex \
	collection.tex \
	process.tex \
	poison_extractor.tex \
	poison_reference.tex \
	evade.tex \
	control.tex \
	tradeoffs.tex \
	propertyview.tex \
	challenges.tex \
	new_future_work.tex \
	future.tex

EPSFIGS = \

EPSGRAPHS = $(wildcard figures/*.eps)

all:   $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) (PAPER)

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

#$(PAPER).pdf: $(PAPER).dvi
#	dvipdf $(PAPER).dvi

# if need to embed font
$(PAPER).pdf: $(PAPER).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out


==> ethics.tex <==
\section{Ethical Tensions}
\label{sec:ethics}

As with any new technology, there are myriad ethical tensions surrounding the
creation of AFR tools. Here, we describe a few. Though resolving these
tensions is beyond the scope of this paper, we believe that
articulating them provides helpful context for future debate.

\para{Privacy vs. National Security.} Innocents and criminals alike
can use AFR tools. Law enforcement's use of facial
recognition can benefit society by catching criminals and
finding lost children, among other use cases \cite{found_child, faceslist}. Consequently, AFR tools
could allow fugitives to evade justice. This debate between privacy and national security plays out in numerous
sensitive domains, such as end-to-end encryption
\cite{doj_e2e}. Legitimate claims can be made by both sides. AFR
researchers ought to be mindful of this debate as they do their work. 

\para{Normalizing Facial Recognition vs. Fighting Status Quo.} A
common criticism of privacy-centric tools (like AFR systems) is that
they tacitly accept society's status quo surrounding personal
privacy. Arguments in favor of AFR tools implicitly acknowledge that
the current lack of online privacy is a fixed rule, rather than a
mutable abberation. Some may even argue that developing
AFR tools disincentivizes regulatory action against facial recognition
(therefore further cementing the status quo)~\cite{savior}. The
tension between legimiate need for privacy {\em now} and the cultural
statement made by developing AFR tools is real. Researchers should be
mindful of this both in how they frame questions of privacy and in the
types of tools they propose.

\para{Evasion vs. Misidentification.} One ethical tension not yet
explored in current literature is the effect of misidentifications
caused by AFR tools. For example, if $U$ uses an AFR tool and is
misidentified by a recognition system as $P$, what outcome might this
have for $P$? If $U$ is engaging in illegal activity but $P$ is
arrested instead, the AFR tool could cause serious harm, both to $P$
and to current/future victims of $U$. It is already
well known that police departments routinely make ill-founded
identification decisions based on partial results from facial
recognition systems~\cite{garbagein}. Furthermore, facial recognition
systems misidentify people of color at higher rates~\cite{gendershades}.
Misclassifications caused by AFR tools could escalate this problem to a new level. 

%\para{Protection Efficacy vs. User Burden.} 



%\para{Performance vs. Accessibility.}




% \shawnc{Ok, I am not an expert in ethics at all. But from a security researcher's perspective, I think this section is not substantial because it only raises questions. Yes, there are hard questions that we cannot answer in this paper, but we should also answer some simple ones to lay the foundation for our discussion. 

% In addition, to discuss under the AI4People framework, I wonder whether we can also borrow some insights from existing privacy toolsets (\eg Tor, end to end encryption). Tor has a blog about ethics that might be interesting (https://blog.torproject.org/category/tags/ethics). Or something more recent and relevant is EU banning the WhatsApp's end-to-end encryption. There are a lot of articles with people taking different sides (privacy vs national security, etc. )

% Again, just some of my wild thoughts, we should ask Ben to take a look at this. 
% }



% The debate surrounding anti-facial recognition technology is fraught
% with ethical land mines. For example, since facial recognition can be used for social
% good (like catching criminals), does this mean AFR tools help individuals but harm society?
% In this section, we raise ethical questions concerning anti-facial recognition tools.

% Since AFR tools are a part of the artifical intelliegence (AI) ecosystem, we develop our questions using the AI4People ethical
% framework~\cite{floridi2018ai4people}. This well-established,
% highly-cited framework names 5 ethical principles meant to
% ``lay the foundations for a `Good AI Society''': {\bf beneficence,
%   non-maleficence, autonomy, justice,} and {\bf explainability}. These principles
% are synthesized from six well-known declarations on AI ethics, including
% the Tenants of the Partnership on AI and the Asilomar AI Principles
% from the Future of Life Institute~\cite{partnership, asilomar}. The
% first four principles are commonly used in bioethics, while the last
% one is added to fit the AI context. %this ethical framework is appropriate. 

% Below, we explain each principle before listing
% related ethical questions about AFR tools. These questions could
% equally apply to the debate about AFR tools as well as specific
% AFR proposals. Though answering these questions is beyond the scope of this
% paper, we believe that articulating them provides helpful context for
% future debate. 

% \para{Beneficence.} The first principle deals with the benefit AFR
% tools provide to society. In the words of AI4People, do they ``promote
% well-being, preserve dignity, and sustain the
% planet?''~\cite{floridi2018ai4people}

% \begin{packed_itemize}
% \item Do AFR tools further human well-being? 
% \item How do AFR tools which require user lifestyle changes (i.e. wearing
%   evasive objects in public or changing one's online persona) impact human dignity? 
% \item Does the computational power needed to implement AFR tools
%   (i.e. generating perturbations via optimization) harm the
%   environment? What about if/when millions of people use these tools?
% \end{packed_itemize}

% \para{Non-malificence.} Beyond beneficence, it is important to
% consider whether AFR tools ``do no harm.'' Even good things
% (i.e. cats) can cause unanticipated harm (i.e. cat dander). This harm
% can be accidental or deliberate. 

% \begin{packed_itemize}
% \item Would AFR tools help criminals evade justice? Would this cause undue societal harm?
% \item Would AFR tools which cause facial recognition systems to
%   misidentify user $U$ as person $P$ harm $P$?
% \item Do AFR tools overpromise the level of real-world protection they provide? Would overinflated perceptions of protection
%   lead users to behave rashly? 
% \item Would democratizing AFR tools incentivize the
%   development of better, more pervasive facial recognition systems? 
% \end{packed_itemize}


% \para{Autonomy.} Autonomy refers to human ability to
% decide for themselves whether they want to use a given AFR tool (or
% AFR tools in general). In creating AFR tools, are we unwittingly
% giving too much power to machines?

% \begin{packed_itemize}
% \item Does the creation of AFR tools tacitly accept facial recognition
% as inevitable? If so, does this harm human autonomy? 
% \item Does the existance of AFR tools reduce societal incentives for
%   regulating facial recognition? If so, does this leave users
%   dependent on AFR tool providers for privacy protection? 
% \item Do AFR tools curtail human experiences (i.e. by requiring
%   cloaking of all online images, etc)?
% %\item Do AFR tools add significant burdens to their users? 
% \end{packed_itemize}


% \para{Justice.} The principle of justice asks whether the benefits of
% AFR tools are universally shared. If AFR tools can only be used by
% certain subpopulations or harm principles of equity, they do not
% promote justice, even if they can protect privacy. 

% \begin{packed_itemize}
% \item Are AFR tools racially biased? Gender-biased? How do we best
%   measure this?
% \item Are AFR tools universally accessible, or is their use restricted to
%   people with certain technological skills or socioeconomic backgrounds?
% \item In general, what new equity issues might common use of AFR tools
%   create? 
% \end{packed_itemize}


% \para{Explainability.} Finally, a common concern in AI ethics is
% whether the actions of an AI tool can be understand and/or
% explained. AFR tools are no exception. If their mechanisms for
% protection are inscrutible, it is worth asking whether they can be
% trusted. 

% \begin{packed_itemize}
% \item Who makes the AFR tools? What are their incentives?
% \item Can AFR tool behavior be understood and explained? 
% \end{packed_itemize}




%%%%%%%%%%%%%%%%%%%% FACIAL RECOGNITION ETHICS QUESTIONS %%%%%%%%%%%%%%%%%%%%

% \begin{itemize}
% \item Unwanted vs unauthorized.
% \item ``Right to be Forgotten'' is good -- what about the ``Right to
%   Public Anonymity?'' This is current allowed in the US, but will that
%   change as facial recognition becomes more prevalent?
% \item 
% \end{itemize}

% Specific questions:

% \begin{itemize}
% \item What does it mean for facial recognition to be unauthorized?
% \item Should AFR tools be used against government systems? Should this
%   be regulated in some way? (i.e. how far does the social contract
%   go?)
% \item Should you be able to opt into a government facial recognition
%   system, the same way you can opt into being an organ donor? I guess
%   the problem with this is that it would increase the chance of
%   misclassification (since there would be fewer people in the
%   system). 
% \item The ethics of misclassifying as someone else in a FR system.
% \item Should police need a warrent to run a facial recognition system
%   on you? (they need a warrant to access much less; i.e. probable cause)
% \item Should you be required to show your face in public?
% \item Since AFR tools require knowledge of where cameras are located,
%   should we require commerical and/or governmental systems to let
%   people know when and where cameras are being used? 
% \end{itemize}



==> future.tex <==
x\begin{table*}
  \centering
%  \resizebox{0.95\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Future Direction} & \textbf{Protection Party} & \textbf{Attack Stages} & \textbf{Limitation Addressed} \\ \hline
Protection with Provable Guarantees & User & $\crc{3}$ $\crc{4}$ $\crc{5}$ & Technical Challenge \\ \hline
Exploiting Camera Artifacts & User & $\crc{1}$ $\crc{5}$ & \begin{tabular}[c]{@{}l@{}}Technical Challenge\\ Usability Challenge\end{tabular} \\ \hline

Tracking Image Use & \begin{tabular}[c]{@{}l@{}}Camera Makers\\ Image Storage/Sharing Platforms\end{tabular} & $\crc{3}$ $\crc{4}$ $\crc{5}$ & \begin{tabular}[c]{@{}l@{}}Power Dynamic\\ Usability Challenge\end{tabular} \\ \hline
Remove Task-irrelevant Information & \begin{tabular}[c]{@{}l@{}}Camera Makers\\ Image Storage/Sharing Platforms\end{tabular} & $\crc{1}$ & Power Dynamic \\ \hline
Permission-Based FR & \begin{tabular}[c]{@{}l@{}}Camera
                                   Makers\\ Image Storage/Sharing
                                   Platforms\end{tabular} & $\crc{1}$
                                                      & Power Dynamic
  \\ \hline
  Legislation & Lawmakers & $\crc{1}-\crc{5}$ & Power Dynamic \\ \hline
  Education & Educator & $\crc{1}-\crc{5}$ & \begin{tabular}[c]{@{}l@{}}Power Dynamic\\ Usability Challenge\end{tabular} \\ \hline
\end{tabular}
 % }
  \vspace{0.1cm}
  \caption{Summary of future directions for AFR tools. }
  \label{tab:future}
\end{table*}

\section{Future Work}
\label{sec:future}

\todo{Synthesize conclucsions from the last two sections here and feed
  those into future work discussion.}

\todo{Also condense this section signficantly.}

\emily{Add section on ``generic future work'' where you discuss the
  ongoing need to address the question of adversarial attacks/defenses
and make adversarial perturbations smaller. These will counteract the
anonymity and usability issues observed in adversarial-example based
AFR techniques.}

The previous section highlights three types of challenges faced
by AFR technologies: power dynamics, technical limitations, and
usability issues. In this section, we consider future work that
could overcome these challenges.

We organize our discussion of future work according to the party who might
deploy it and note which stage(s) of AFR it affects. Different parties can more effectively target
different stages and address different challenges. For example, online platforms hold greater sway over
stage $\crc{1}$ AFR efforts, since they manage online
content and can help shift the balance of power. However, individual
people can best deploy real-time AFR methods, such as stage $\crc{5}$
evasion, since they can take a more flexible approach to deploying AFR
tools than would a beaurocractic organization.  

First, we consider future work at the {\bf user level}, which
could help overcome technical and usability issues of current AFR
proposals. Then, we discuss how {\bf third-party entities} like camera
makers and online platforms could support AFR technologies, helping
shift the power dynamic and increase tool usability. Finally, we
address {\bf legislative efforts} which could change how facial recognition
is used. A summary of future work, along with the stages affected and
challenges addressed, is in Table~\ref{tab:future}.

% Next, we identify several future directions of AFR technology that we think are under-explored and promising. 

% We first discuss potential legislative efforts that might change the tide of
% AFR discussion. Then we introduce the parties that can deploy 
% AFR technology and the pros and cons to deploy by each party. 
% In the end, we discuss several research directions that might produce
% effective AFR technologies. 

\subsection{User-Level Future Work}

Most current AFR proposals are designed
to be deployed by individual users. While user-level tools cannot
address the power dynamic problems of AFR proposals, they can be
improved to address technical and usability issues. To this
end, we believe future user-level AFR proposals should work towards
providing provable protection guarantees for users and exploiting camera
artifacts.

\para{Protection with Provable Guarantee.} Nearly all AFR proposals lack provable
  guarantees, meaning that future adaptations could compromise all
  past protection~\cite{savior}. The only exception~\cite{identitydp} uses differential privacy, which can provide a
  mathematical guarantee of anonymity. However, this proposal
  changes users' physical appearance in photos, rendering it unusable
  in practice. Methods with privacy guarantees such as differential privacy~\cite{dwork2014algorithmic,
abadi2016deep} and K-anonymity~\cite{sweeney2002k} have been widely
studied in the privacy literature and could be used in AFR tools,
especially those targeting stages $\crc{3}-\crc{4}$. Future proposals
aimed at the user level should aim to incorporate provable protection guarantees.  % Most of existing AFR tools offer no 
% privacy guarantee which leads to user's privacy being compromised. Apply some of the techniques with
% guarantees is a natural next step for AFR techniques. 

\para{Exploiting Camera Artifacts.} Many user-level AFR
  proposals target physical image capture but assume cameras capture
  images perfectly. In practice, cameras have many artifacts which
  could be exploited to improve AFR efficacy. For example, most modern cameras have a rolling shutter
  effect~\cite{liang2008analysis} that add artifacts to images. Recent work~\cite{sayles2021invisible} leverages 
  these artifacts to construct adversarial examples which fool neural
  networks. Similar techniques could be used in AFR. Highly reflective
  clothes could also degrade the quality of images, making these an
  interesting option for AFR proposals. It remains unclear how
  easily camera-based artifacts can be removed from images, either by changing shutter
  speeds or post-processing techniques. Future work should assess the
  effectiveness and robustness of artifact-based AFR techniques. 


\subsection{Third-Party Future Work}
Existing AFR tools assume protection takes place at the user level (\eg
users compute perturbations for their images or wear protective clothes). 
However, since $A$'s goal (typically) is to identify as many
people as possible, cooperation among users would greatly enhance
the efficacy of AFR tools. This possibility has been noted in several AFR
proposals, such as the ``group cloaking'' in Fawkes~\cite{fawkes} or
cooperative reference database poisoning in FoggySight~\cite{foggy}
Existing proposals require users to manually coordinate their
efforts, a daunting prospect as the number of users increases. Future
work should explore how third parties like \emph{image storage/sharing
  platforms} and \emph{camera makers} can help scale AFR proposals. We
describe these parties and then their potential contributions.


% introduces a group cloaking technique where users
% can cooperate to achieve higher protection
% rates. FoggySight~\cite{foggysight} suggests similar cooperation to
% corrupt A's reference database. Data
% leverage~\cite{vincent2019data,dataleverage} requires user cooperation
% achieve its effect.

% computing evolves, this challenge will diminish.

{\em Image Storing/Sharing Platforms.} After face images are captured, they are often 1) stored in 
local (\eg Android Gallery) or cloud devices (\eg Dropbox), or 2) 
shared through applications (\eg Firefox) or websites (\eg Twitter, Flickr). 
These platforms have already demonstrated interest in protecting user 
privacy in other domains~\cite{appleupdate,googlefloc}. Some have specifically fought back
intrusive facial recognition systems (\eg by sending cease-and-desist orders to
companies like Clearview.ai~\cite{fb_cease}). They could further
curtail unwanted facial recognition by deploying AFR
techniques at scale.

{\em Camera Makers.} Cameras play a huge role in facial recognition
because they capture face images. AFR tools deployed at the camera level
(hardware or software) can impact all downstream facial recognition
tasks. % The challenge of deploying AFR tools in cameras is
% computational overhead of current AFR techniques, but as edge



% There are many benefits of deploying AFR on these platforms. First, many of the system 
% have a global view of many user's face images, which is helpful in generating protection
% and monitor protection effectiveness
% as presented by several existing AFR techniques~\cite{vincent2019data,dataleverage,fawkes,foggy}. 
% Second, many of these platforms are large and technology companies that have the extra resources and
% expertise in implementing AFR tools. 

% \para{Educators. } User awareness is crucial in privacy technology. Educators can make a difference
% by educating face privacy to the younger generation who do not have as much of an online presence. \shawnc{I personally think educator is a bit boring. Like that is something people have already know. }

\para{Limiting and Tracking Image Sharing.} Because online platforms
host face images from many users, they could easily implement
protection mechanisms and track the efficacy of that protection.

\textit{Privacy-aware Image Sharing: }  While many image platforms use
 anti-scraping defenses, few provide privacy protection at the
 individual image level. The sensitivity of face images and known
 (ab)use of images scraped from image platform demands that platforms
 devote more effort to protecting image privacy. For example,
 platforms could employ the group cloaking techniques of
 Fawkes/FoggySight to obscure user characteristics in scraped data. These privacy-preserving techniques ought to be
accompanied by enhanced anti-scraping techniques designed to
prevent large-scale scraping of face images, \ie stricter rate
limiting, access permissions, and scraping detection heuristics.  

\textit{Tracking Data Provenance:} Even if images are scraped, image-sharing platforms
could use provenance-tracking techniques to re-identify stolen images,
e.g. in the training dataset of a feature extractor. This provenance tracking would allow the user or platform
to take legal action against the image thief. Preliminary work
% on membership inference (i.e. identifying if an image is in a training
% dataset)~\cite{} and
% radioactive data (i.e. causing data to ``mark'' a model during
% training)~\cite{radioactive}
shows such provenance-tracking is
possible~\cite{salem2018ml,shokri2017membership, radioactive}. However, these proposals make impractical assumptions (\ie
\cite{radioactive} requires controlling $>20\%$ 
of the training data), provide no formal guarantees that could stand in court%  (\ie membership
% inference tools offer no formal guarantees)
, and can be thwarted by countermeasures~\cite{jia2019memguard,ying2020privacy,chen2020differential,chen2020differential}. Despite
these limitations, future work on image provenance tracking could limit
attackers' ability to steal images without consequence.


\para{Removing Task-irrelevant Information. } Face images can include an abundant amount of 
\emph{task-irrelevant} content that leak unnecessary 
information. Task-irrelevant content includes content that is irrelevant for intended
use of the image (\eg bystanders in a selfie) or redundant (\eg video
stream of a customer taken by a theft detection camera or a traffic violation camera). 
These task-irrelevant content contains rich data for any facial recongition that can be used to 
create reference database or as query images. Removing this
content can significantly reduce the amount of data available to
$A$ and protect privacy. Although users could remove this information
manually in some cases, camera makers or online platforms could do so at scale, lowering cost
and increasing efficiency.

{\em Removal via Classification.} One way to remove task-irrelevant information is to filter it out
using an ML classifier that predicts which information is relevant. Existing work~\cite{hasan2020automatically} has explored using a neural network
to remove bystanders from surveillance videos. Similar techniques could
be applied to other types of content removal, like saving only the
theft footage from security cameras.

{\em Removal via Information Bottlenecks.} Information bottlenecks
restrict information flow to only include the necessary information while discarding the rest. In the context of face images, such bottlenecks
can be used to remove information in images that is not useful for training a
machine learning classifier. A straightforward way to use information
bottlenecks for AFR purposes would be to include an additional
loss function during model training to ignore irrelevant information
in face images. Similar techniques have already been used to defened
against adversarial attacks~\cite{wu2020graph,liu2020defending}.



\para{Permission-Based Facial Recognition. } Privacy laws to offer users the option to opt-out certain types of 
tracking (\eg online cookies and tracking, biometric data
collection)~\cite{gdpr}. While no existing legislation yet requires similar opt-out
options for unwanted facial recognition, this model could prove
effective. However, unlike other types of tracking (\eg cookies), it is hard to implement a 
opt-in method for real-time facial recognition.  Such a method would
require cameras to distinguish between opt-in users and opt-out users
in real time. If camera-makers could implement this, it would
support future legislation requiring permission for facial recognition.

One way to manage permissions at the camera level would be to have
cameras emit signals to communicate with mobile phones. These signals
could notify users that cameras are present and request image-capture
permission. A user could manage tracking permissions on their phone,
potentially enabling tracking for certain types of cameras while
opting-out of others. If the user opts out, the camera could locate
the user using their phone coordinates and blur the user's face. 

This approach requires edge cameras to communicate
permission options, identify users, and blur images -- a heavy
computational burden. Other more centralized approaches 
are possible. For example, the camera maker could remove all opt-out
users' faces after image capture. However, this approach assumes an
honest camera maker and still requires users to have their face images
captured by the camera even when they are opt-out (before the images
are blurred by the server.)


\subsection{Legislative Future Work}

Legislative efforts could augment user- and system-level AFR
  proposals. Regulations surrounding data use, such as GDPR, and facial
  recognition are increasingly common but far from ubiquitous.
 For example, Canada declared Clearview.ai to be illegal and demanded
 that the firm delete facial images of Canadian citizens from its
database~\cite{canada_nyt}. Clearview.ai also faces a slew of
lawsuits from California, the European Union, and others, while being investigated by Britain and Australia for its use of citizens' personal information~\cite{clearview_money}. Although companies like Clearview are fighting back against 
these regulations, facial recognition is likely be more heavily
regulated in the future. Even China recently passed a bill requiring
commercial companies to obtain users' consent before performing facial
recognition~\cite{china_ban_commercial}.

While efforts to regulate facial recognition are promising,
historical precedent shows that legislation can only go so far. First
and foremost, such legislation is hard to enforce. 
Even after GDPR banned online tracking after a user has opted-out,
around half of websites never stopped tracking users or resumed tracking
after a brief pause~\cite{sakamoto2019after}. Second, legislation is
open to interpretation. Both GDPR and CCPA (California's privacy law)
mandate specific disclosure when surveillance cameras are in use, but they do
not specify how people should be notified about the cameras. This
inevitably led to poor follow-through by companies~\cite{zhang2021did}.

While effective, legislative efforts are limited by geopolitical regions,  
implementation concerns, and delayed reaction time. As a result, legislative efforts alone are not 
sufficient to address the privacy concerns of facial recognition in the near future. This leaves a
crucial gap which must be filled by AFR tools.




==> limitations.tex <==

\section{Tensions and Challenges}
\label{sec:limits}

While existing anti-facial recognition tools have proven successful in
constrained lab settings, their use in the ``real world'' faces
numerous obstacles. Here, we consider the ethical tensions
and implementation challenges for AFR tools. 

\subsection{Ethical Tensions}
\label{subsec:ethics}

As with any new technology, there are myriad ethical tensions surrounding the
creation and use of AFR tools. Here, we describe a few. Though resolving these
tensions is beyond the scope of this paper, we believe that
articulating them provides helpful context for future debate.

\para{Privacy vs. National Security.} Both privcy-sensitive citizens and criminals
can use AFR tools. Law enforcement's use of facial
recognition can benefit society by catching criminals and
finding lost children, among other things \cite{found_child, faceslist}. Consequently, AFR tools
could allow fugitives to evade justice. The debate between privacy
and national security plays out in numerous other tech domains, such as end-to-end encryption
\cite{doj_e2e}. Legitimate claims can be made by both sides. AFR
researchers ought to be mindful of this debate and this tension and
the potential consequences of their work.

\para{Normalizing Facial Recognition vs. Fighting Status Quo.} A
common criticism of privacy-centric tools (like AFR systems) is that
they tacitly accept society's status quo surrounding personal
privacy. Arguments in favor of AFR tools implicitly acknowledge that
the current lack of online privacy is a fixed rule, rather than a
mutable abberation. Some may even argue that developing
AFR tools disincentivizes regulatory action against facial recognition
(therefore further cementing the status quo)~\cite{savior}. The
tension between legitimate need for privacy {\em now} and the cultural
statement made by developing AFR tools is complex. %  Researchers should be
% mindful of this both in how they frame questions of privacy and in the
% types of tools they propose.

\para{Evasion vs. Misidentification.} One ethical tension not yet
explored in current literature is the social effect of misidentifications
caused by AFR tools. For example, if $U$ uses an AFR tool and is
misidentified by a recognition system as $P$, what outcome might this
have for $P$? If $U$ is engaging in illegal activity but $P$ is
arrested instead, the AFR tool could cause serious harm, both to $P$
and to $U$'s victim(s).

The well-known bias of FR systems heightens this tension. Police
departments routinely make ill-founded identification decisions based
on partial results from facial recognition
systems~\cite{garbagein}. Furthermore, facial recognition systems
misidentify people of color at higher
rates~\cite{gendershades}. Recent work has found that AFR tools
exhibit these same biases~\cite{rosenberg2021fairness,
  qin2021bias}. The social impact of AFR misclassification requires
urgent study. \emily{It may be the case that stricter regulation of
  FR systems, in light of the knowledge that they will produce
  misclassifications and false positives, is the only reasonable solution.}

\subsection{Implementation Challenges}
\label{sec:challenges}

Beyond ethical tensions, AFR tools also face implementation challenges. Some challenges stem from the {\bf power dynamics} in the world at large, others relate to {\bf technical
  challenges}, and some arise from {\bf usability challenges} of
current AFR tools. In this section, we examine challenges under these three
headings. The goal is to provide insight into how these challenges
arise and how/if they might be overcome.

\para{Power Dynamics:}

{\em 1) Adversary unregulated and unpredictable:} There
are few legal regulations surrounding the use of facial
recognition. Consequently, it is difficult (if not impossible) for
individuals to know when facial recognition systems are
deployed and what they are capable of. This difficulty is compounded by the fact that law
enforcement and other governmental bodies have eagerly adopted facial
recognition, reducing internal governmental pressure to regulate FR. A
few recent legislative efforts are pushing back, such as the Illinois Biometric Information Privacy Act~\cite{bipa}
and China's facial privacy decree~\cite{china_ban_commercial} but general regulation of FR technology is
elusive.


\para{Technical Issues:}


{\em 1) AFR tools protect static data.} For better or
for worse, most people have the same face their whole life~\footnote{Major
plastic or reconstructive surgery excepted.}. Our faces change as we
age, but they remain recognizable as uniquely ``us'' to most
humans. Prior work shows that FR accuracy remains high
 even with a $10$ year age gap between the reference and test
images~\cite{ling2009face}. The slow rate at which faces change is a
major challenge for AFR tools. To be long-term effective, these tools
must conceal the same piece of static data (a face) from numerous
adversaries over many years. 

{\em 2) No provable protection guarantees.} Unlike
cryptographic techniques, AFR tools lack formal mathematical
guarantees of protection. Consequently, it is unsafe to assume they
are future-proof. Rayni-Dixit and Tramer discuss
extensively how techinques used to evade facial recognition may cause
users to have a false sense of security~\cite{savior} due to the
potential of future compromise. Other privacy
protection mechanisms also lack such guarantees (\ie protection based
on hard problems which are no longer hard under new computing paradigms, e.g. quantum crypto ~\cite{attema2021post}). Face data is even more vulnerable once exposed because it changes so slowly. 

 {\em 3)  Defenses thwart adversarial perturbations.} Many AFR tools
 rely on adversarial perturbations to fool object detection or facial
 recognition models. Defenses designed to thwart generic adversarial
 examples can also defeat AFR tools. For example, adversarial training
 may mitigate the effect of cloaked data in the extractor training or
 labeled image database creation process~\cite{oriole, savior}. Other
 defenses claim they remove adversarial perturbations (such as
 those designed to thwart face detection)~\cite{faceguard}. Defenses
 against adversarial examples are an active area of research and may pose a problem for AFR tools.


\para{Usability Quandries:}

{\em 1) Privacy/usability tradeoff.} The tradeoff between usability
and privacy has been well-studied in other
domains~\cite{acquisti2016economics, coopamootoo2020usage,   wright2002privacy}. Proposed AFR methods such as participating in
data leverage activities, wearing strange patterns on clothes, or
adding perturbations to online images place additional burdens on
users. Preliminary user studies show that users are willing to add
visible perturbations to online images in order to evade
recognition~\cite{faceoff}, but no study has confirmed user
willingness to engage in other, arguably more obvious, AFR behaviors.

{\em 2) People already have online footprints.} A
major usability challenge of proposals designed to protect {\em online
  images} is that many people already have an online footprint.%  Even those
% without an intentional online footprint cannot completely control
% which images of them are posted online, perhaps by well-meaning
% friends documenting an event they attended. 
% Online labelled facial images of a user could be
% added to a reference database and used for future recognition a la
% Clearview.ai~\cite{clearview}
State-of-the-art facial recognition
systems only require one clean picture to create a reasonable feature
vector for the $U$~\cite{arcface}. \shawn{For example,
  Clearview.ai identified a child abuser using a single reference
  image in which the abuser's reflection appears faintly in a mirror~\cite{hill_clearview}.  Given the online
  nature of life today, completely eliminating online's footprint is a
  difficult task.}

{\em 3) Accessibility gap.}  The final usability challenge of AFR
tools is the large gap between the people {\em able} to use such tools
and the people who {\em want} to use them. Of all existing AFR
proposals, only two~\cite{fawkes,lowkey}, have made a substantive
effort to make their tool available to the general public\footnote{And
even still, these tools assume users have relatively powerful computers
with uncensored internet connections}. This means that people without
  sophisticated technical knowledge are effectively barred from using
  most current AFR tools, but those who are tech-and-privacy savvy
  can use them. However, such people likely possess significant social and economic capital, making AFR tools less pivotal for
  their protection. % This disconnect from the public is a problem for
  % academic research in general, and it is particular painful for
  % high-stakes situations like avoiding unwanted facial recognition. 


%\subsection{Limitations of Attacking Specific Stages}

% \begin{table*}
%   \centering
%   \resizebox{0.95\textwidth}{!}{
%   \begin{tabular}{|c|l|l|c|c|} 
%     \hline
%     \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Attack
%         }\\\textbf{Stage}\end{tabular}} &
%     \multicolumn{1}{c|}{\textbf{Ideal Use}} & \multicolumn{1}{c|}{\textbf{Limitations}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Protection }\\\textbf{Usability}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Protection}\\\textbf{Efficacy}\end{tabular}} \\
%     \hline
%     $\crc{1}$ & Prevents collection of labelled training/database images. &  Requires third-party support or control of online identity.  &  High & Yes \\
%     $\crc{1}$ & Prevents capture of unlabelled query images. & Assumes knowledge of camera location and use. & Low & Yes\\
%     $\crc{1}$ & Thwarts successful face detection. & Assumes knowledge of camera location/face
%     detection model. & Low & Yes \\
%     $\crc{1}$ & Anonymizes user identity in labelled images. & Anonymized images do not resemble user. & Low & Yes \\
%     $\crc{2}$ & Poisons extractor training. & Identity information not retained after training. & High & No \\
%     $\crc{3}$ & Prevents identity creation. & May result in misclassification as another person. & Medium & Yes \\
%     $\crc{4}$ & Evades successful detection. & May result in misclassification as another person. & Low & Yes \\
%     \hline
%   \end{tabular}
%   }
%   \vspace{0.1cm}
%   \caption{\todo{cut?} Summary of pros/cons of attacking at each interaction
%     stage. All descriptions provided are in terms of
%     protection provided by ideal attack at this stage. \todo{Change
%       the key for this table so it is keyed by limitation rather than stage?}}
%   \label{tab:pros_cons}
% \end{table*}

% \subsection{Summary Thoughts}
% TBD -- idea is to summarize all the limitations here.
% \emily{@Shawn -- maybe we could address the results from Table 8
%   here?}

%%%%%%%%%%%%%%%%%%%%   TEXT GRAVE %%%%%%%%%%%%%%%%%%%%

% decree that commerical entities must obtain user consent before deploying
% facial recognition,

% This lack of regulation has several practical consequences for
% users. First, the location of facial recognition cameras are unknown. % $\crc{2},\crc{3},\crc{7}$.} Three key
% This makes techniques to avoid real-time image captured (stage
% $\crc{1}$) nearly impossible in practice. % assumptions underpinning proposals to thwart {\em real-time image capture}
% are that a user knows (1) {\em where cameras are located} (2) {\em when/if
%   a facial recognition model has been deployed} and (3) {\em if so, which
%   model it is}. With this presupposed knowledge, $U$ can don the
% appropriate evasion gear -- i.e. a hat, special glasses, etc. -- and
% either prevent proper image capture or evade the model. In practice,
% these assumptions are unrealistic. As~\cite{china_artist}
% shows, government and corporate security cameras can be added or moved
% without notice. Thus, avoiding them completely requires
% preternatural knowledge about building and street schematics.
% If a user wishes to avoid detection using these physical avoidance methods
% but doesn't know where the cameras are, they must default to wearing the
% evasion gear all the time. This places an undue burden on the user.

% Second, $A$'s adaptations are also unknown to users. For example,
% during the COVID-19 pandemic, widespread mask wearing led facial
% recognition providers to adapt their algorithms. Now, wearing a face
% mask (a previously recommended evasion technique) is ineffective to
% avoid detection. This adaptation only came to light because of a
% report from NIST in early 2021, which found that numerous commercial facial
% recognition systems can now identify mask-wearers with high
% accuracy~\cite{nist_mask}. Without this report, individual users would
% not know that masks cannot protect their identity.


% {\em Attacking stage $\crc{1}$} can thwart successful image capture,
% but has some specific limitations. First, facial recognition may be powerful
% enough to overcome generic mask-wearing and other more general face
% obfuscation techniques. In early 2021, NIST reported 
% Additionally, depending on the context in which $U$ wishes to evade image capture, their actions may raise human
% suspicion. Wearing a mask, hat, or other obfuscating clothing could
% attract the attention of nearby observers, who make take note. 

% \para{Power Dynamic 2: Flow of money favors adversary.} Today, far more
% money is spent collecting people's data than is spent protecting
% it. The modern economy is built on the presupposition that data,
% including facial images, is free for the taking and can be resold for profit~\cite{surveillance_capitalism}. Tech companies make billions of
% dollars every year by harvesting and selling individuals'
% data~\cite{guardianreport}. While some academic programs invest significant
% funds in developing privacy-centric tools, money generally flows in
% the opposite direction. Consequently, developing privacy-centric
% tools, like AFR tools, is an uphill battle.


% However, it is worth
% noting that evading a FR system in which one's identity is
% already enrolled is in many ways a last ditch effort. Attacking this
% point in the pipeline means that there are no other protection
% mechanisms in place, so failure here could be catostrophic. An
% additional area of concern here is the possibility that query images
% are fed back into the gallery. This means that evasion techniques
% cannot be static (i.e. same perturbation used again and again),
% otherwise the system may be able to develop a profile based on the
% specific evasion pattern and begin to recognize the individual.

%% \para{Possibility of Non-machine Corroboration.} Evasion techniques,
%% with their highly visible and suspecious evasion methods, also
%% presuppose that there is no human present who could point out the
%% strange objects and request their removal. Such assumption is likely
%% not hold in certain scenrios (\eg TSA officer requests a person to
%% remove adversarial mask).


%% \para{Potential Probe Re-use.} It has not yet been studied if evasion
%% examples can also function as poisoning examples for feature vector
%% creation. Given the ambiguity around data re-use in FR systems.



%\para{Selling Data is Profitable $\crc{1}-\crc{7}$.} 
%\para{Image Capture is Sometimes Mandatory $\crc{1} - \crc{7}$.}
% \subsection{Technical Limitations}
% \label{sec:general_limits}
% \emily{Nature and culture create structural limitations for AFR
%   tools. However, there are also technical limitations that should be
%   noted. In this section, we discuss technical limitations which
%   affect multiple attack stages. The next section deals with
%   stage-specific technical limitations.}
% Anti-facial recognition tools face numerous challenges in their
% deployment and potential success. Here, we discuss these common
% challenges, starting from the most fundamental and working down
% towards more specific implementation issues. We note the specific
% stages impacted each by limitation.

%covers one incidence of unprotected or poorly protected face
% image of a user at any point in time, it becomes extremely challenging for the user 
% to avoid FR.
%\para{AFR Tools Burden Users $\crc{1}-\crc{7}$.} 
%that has high cost but low guaranteed rewards. }

%% However,
%% obtaining a driver's license or other ID is a fundamental requirement
%% for most citizens of any country, as it enables society to function
%% smoothly.

%% The authors of Fawkes~\cite{fawkes} indicated on their
%% public website that this adversarial training may have occured in the
%% wild. After Fawkes code had been publicly released, the authors found
%% that their cloaking techniques were no longer effective against
%% Microsoft Azure, which may have employed adversarial training
%% techniques.

%% \para{Poisoning is Non-Adaptive.} \cite{savior} discusses extensively
%% the security game of data poisoning attacks. In this setting, the
%% "attacker" (aka the user) goes first, and is then incapable of knowing
%% how their attack performs until something big happens. Because the
%% attacker always goes first, and the defender has their data for all
%% time (assuming it is scraped), if the cloaking mechanism doesn't hold
%% up, then the user cannot adapt. Their data is already gone. A few
%% preliminary works ~\cite{savior, oriole} have demonstrated training
%% techniques that could render cloaking useless.



% Having considered the more fundamental social and technical limiations
% of AFR tools, we now consider limitations of deploying AFR tools at specific stages. We organize our analysis, as before, according to the
% interaction stages of Table~\ref{tab:points}, but we skip over stages
% for which we have identified no specific limitations. % The pros/cons are
% % summarized in Table~\ref{tab:pros_cons} and are expounded upon below.

% \para{Stages $\crc{1}-\crc{4}$.}

% {\em  Attacking stage $\crc{1}$} requires either an immense amount of
% control over one's online identity or the assistance of 3rd party
% entities (i.e. anti-scraping). However, if possible, protection at
% this stage is arguably more powerful than at any other
% stage. % Preventing collection of training or gallery data is a great
% way to ensure you never end up in a model.



%{\em Attacking stage $\crc{1}$} has no additional limitations. % beyond those noted in \S\ref{sec:general_limits}. % and those related to
% physical evasion techniques, as discussed in the prior paragraph. If effective, this method
% prevents data from leaving the preprocessing pipeline. This, again,
% cuts off facial recognition at the root by rendering data unusable.



% \para{Stage $\crc{2}$.} The fundamental problem with attacking at
% Stage $\crc{2}$ is that {\em identity information is not retained
%   after extractor training ends.} Feature extractor
% training is meant to produce a model which maps different faces into
% different parts of an $N$-dimensional mathematical space. % This mapping
% % process can be used to quickly identify people in new pictures by comparing against
% % a database of such mappings (see Fig.~\ref{fig:dataflow}). 
% Therefore, poisoning identity creation at this stage will not achieve the desired
% result (i.e. avoiding recognition).

% \para{Stage $\crc{3}$.} Identity corruption techniques are a high-risk, high-reward
% prospect. If successful, these methods allow users to erase themselves
% from the model by poisoning the gallery dataset. However, as noted
% in \S\ref{sec:general_limits}, these methods are ineffective if
% unprotected user data is already present in the gallery. A few works \cite{fawkes, lowkey} have proposed
% communal cloaking methods that could limit the effect of unprotected images. However, as~\cite{savior} points out, an
% attacker could simply adjust the time frame of their scraping to avoid
% capturing images that could be cloaked. % Furthermore, using
% identity-protection mechanisms means that a user's profile in the
% gallery is associated with an incorrect identity, meaning that the
% either the user is recognized as someone else, and someone else is recognized as the user. This is a
% yet-unexplored ethical concern that needs to be investigated.
%\para{Stage $\crc{4}$.} There are no additional limitations of attacking at this stage. 

% {\em Attacking stage $\crc{1}$} using anonymization methods severely
% distorts users' appearance, typically to the point of being unrecognizable by humans. While this distortion does accomplish the
% goal (anonymity), it comes at the cost of usability.  Users who post photos on social
% media often do so because they want to showcase their activities to
% friends. Putting up images of someone who barely resembles themself
% may defeat the purpose. Furthermore, Recent work from Stadler et al call into
% question the privacy-preserving capabilities of differentially private
% training data (a la~\cite{identitydp})~\cite{stadler2020synthetic}. They find that the lack
% of clarity about which traits DP actually hides may obscure flaws in
% the protection mechanism. 


%% NOTE: Emily commented this out bc Nick Vincent pointed out that
%% these studies really only measure users' value of privacy "assuming
%% nobody else does anything". This might not be the case here.

% Current AFR tools require significant time, energy,
% and diligence from users in order to ensure proper functioning. \shawn{Average
% users place low value in their privacy as shown by Tan \etal~\cite{tan2018comparing},
% who found that users would be willing to sell their physical location
% informaation to an advertising company for less than $10$ USD. Thus,
% it is unclear how many users will be willing to employ AFR techniques,
% which offer few guaranteed rewards at a high use cost.}


==> new_future_work.tex <==
\section{\bf Open Challenges of AFR}
\label{sec:future}

% An ideal AFR tool should guarantee {\em ongoing anonymity}, be
% implemented in a {\em  privacy-preserving} manner, place a {\em
%  minimal burden} on users, and would ideally be {\em user-centric}. The prior section analyzed if (or to what extent) AFR
% tools operating at each stage meet these criteria. Here, we extend
% this analysis to consider broad challenges for AFR researchers.

We describe here what we see as four major challenges facing AFR 
development. Each of these challenges spans multiple properties and
stages laid out in this paper. For each challenge, we provide context for why the challenge
exists and, where possible, suggest ways to address it. Like \S\ref{sec:tradeoffs}, the challenges described here represent our
best efforts to understand and systematize the AFR space. They are not
exhaustive, and are meant as signposts rather than a comprehensive map for
future research. 

%  In the top table of Figure~\ref{fig:challenges}, properties which could be (but are not yet) achieved by current
% AFR proposals are marked by $\gcirc$. This section considers future
% work which could turn those $\gcirc$ into $\fcirc$, i.e. allowing AFR
% tools to achieve the particular property. For each of the four
% properties (anonymity, usability, autonomy, ongoing protection), we
% outline key challenges impacting AFR tools' ability to achieve the
% property and propose future work to overcome these challenges. These
% challenges are summarized in the bottom of Figure~\ref{fig:challenges}
% and explained in detail below.

\noindent\rule{\linewidth}{0.4pt}
{\bf Challenge 1: Lack of provable protection} \\
\noindent\rule{\linewidth}{0.4pt}

 %\para{Background.}  

Our analysis shows that the majority of AFR proposals, especially those targeting stages
  {\bf $\crc{2}-\crc{5}$},  employ adversarial
  perturbations, which do not yet provide provable protection
  guarantee.   In practice,  the success rate of adversarial
  perturbations may drop largely when \pr's knowledge of \adv~is imperfect~\cite{demontis2019adversarial}.  Many adversarial perturbation-based protections can also be
  circumvented by more advanced FR systems. For example, \adv~could
  adversarially train the feature extractor~\cite{oriole, savior} to
  be more robust against adversarial examples,  thus defeating AFR
  tools against stages $\crc{3}$ or $\crc{4}$.  \adv~could also remove adversarial
  perturbations from face images before entering them into the
  recognition system~\cite{faceguard}, which disrupts AFR tools
  targeting stages $\crc{2}$ or
  $\crc{5}$. 


% This has two major implications for AFR
%   tools. First, AFR tools are not guaranteed to work in
%   the first place, as adversarial attack efficacy can be
%   strongly affected by small discrepancies between the AFR tool and
%   its target~\cite{demontis2019adversarial}. Second, AFR protection
%   can be circumvented, as defenses against generic adversarial perturbations can defeat AFR tools. For example, \adv could adversarially train their feature extractor (defeating stage $\crc{3}$ or $\crc{4}$ tools)~\cite{oriole, savior} or remove adversarial perturbations from images before classification (defeating
%   tools targeting stages $\crc{2}$ or
%   $\crc{5}$)~\cite{faceguard}. 

%\para{Key Insights.}  

\para{Potential Directions.}  Improving adversarial perturbation generation
methods may help improve short-term efficacy of those AFR
tools. However, the lack of provable, ongoing
protection is a much tougher barrier to overcome. 
%Other privacy
%protection mechanisms also lack such long-term guarantees (\ie quantum
%computers will render existing cryptography obsolete~\cite{attema2021post}). However, face data is even more vulnerable
 % if exposed because it changes so slowly~\cite{ling2009face}. 
In order to provide reliable, ongoing protection, developers of AFR
tools can 
consider two possible paths: 
(i) integrate provable guarantees into the perturbation generation
process, or (ii) consider an alternative method that provides
guaranteed protection.  For (ii), there are two potential directions.  The first is to add more efforts on attacking stage $\crc{1}$,
where defeating FR does not require tackling a feature extractor.  The
second is to switch from ``misleading'' the feature extractor with
``minor'' image modifications to completely disabling the feature
extraction and/or matching process.  

%Along this line,  a viable
%direction is {\em Integrating cryptographic techniques}
 % such as differential privacy~\cite{dwork2014algorithmic, abadi2016deep} and
%K-anonymity~\cite{sweeney2002k} into AFR tools, especially for those targeting stage
%$\crc{4}$. 


% {\em Depending less on adversarial
%     preturbations} could take one of two forms. It could mean shifting
%   AFR efforts to stage $\crc{1}$, where avoiding FR does not require
%   evading/poisoning a feature extractor. Alternatively, it could mean developing tools which
%   block FR systems completely at later stages (e.g. via lights shined on surveillance
%   cameras, etc) rather than attempting to fool the feature extractor
%   with image modifications.  {\em Integrating cryptographic techniques}
%   such as differential privacy~\cite{dwork2014algorithmic, abadi2016deep} and
% K-anonymity~\cite{sweeney2002k}, into AFR tools could also help address
% this problem, especially for AFR tools targeting stage
% $\crc{4}$. Regardless of technique, future AFR proposals should
% incorporate provable protection guarantees in order for protection to
% be trustworthy and meaningful.

% {\em Solution: Decreased reliance on adversarial perturbations
%   $\crc{2}, \crc{4}, \crc{5}$.}
% Given the ongoing competition between adversarial attacks and
% defenses, future AFR tools may be best implemented through other
% mechanisms. This would circumvent the constantly shifting winds of
% adversarial machine learning. Potential targets for future work
% include fundamental properties of models outside the feature space. 


\noindent\rule{\linewidth}{0.4pt}
{\bf Challenge 2: Existence of online footprints}\\
\noindent\rule{\linewidth}{0.4pt}

AFR proposals (especially those targeting stage $\crc{4}$) often 
assume that individuals have complete control over their online photo
footprint, and can modify online images of themselves, past and
future.  In practice, this is impossible.  As over 1.8 billion photos
are uploaded to online platforms daily~\cite{forbes_photos},  one or
more unmodified photos of a user \pr~will likely end up online without
\pr's knowledge and/or 
consent.  Unfortunately, modern FR systems only need one clean
picture in the reference database to identify a
person~\cite{arcface}.  For example, Clearview.ai identified a child
 abuser based on a single reference image in which the person's reflection appeared faintly in a mirror~\cite{hill_clearview}.

% AFR proposals aimed at securing one's online photos
% against unwanted FR (e.g. stage $\crc{4}$) require that individuals have complete control over their online
% footprint. Most proposals asssume individuals can modify all online
% images of themself, past and future, that could possibly end up in a
% FR system. In practice, this is impossible. Over 1.8 billion photos
% are uploaded to online platforms daily~\cite{forbes_photos},
% making it likely that a photo of \pr~ends up
% online without their consent. Modern FR systems only
% require one clean picture in the reference database to identify
% \pr~\cite{arcface}. For example, Clearview.ai identified a child
%  abuser using a single reference image in which the abuser's reflection appeared faintly in a mirror~\cite{hill_clearview}.% to create a reasonable feature vector for
% % the $U$~\cite{arcface}. 

\para{Potential Directions.} 
This stark reality casts two implications on future AFR research. 

{\em First}, 
we believe that AFR tools administered by online platforms will offer a tighter
protection of our online footprints against FR systems than those executed by individual
users. However, this is at the cost of potential loss of user privacy
and agency.  For example, online platforms could employ the 
 group cloaking techniques proposed in Fawkes or
 FoggySight~\cite{fawkes, foggy} to corrupt reference databases
 composed of images from their sites.  And after images are scraped,
 online platforms could use provenance-tracking to re-identify stolen images,
{\em e.g.\/} in the training dataset of a feature extractor, and enable
exposure/prosecution of photo thieves~\cite{salem2018ml,shokri2017membership,
  radioactive}. All these methods ought to be accompanied by
enhanced anti-scraping techniques to prevent large-scale scraping of face images, \ie stricter rate limiting, access permissions, and
 scraping detection heuristics, to make it safer for individuals to
 have online footprints.





  {\em Second}, AFR tools should be evaluated under the practical 
scenarios where the FR system has access to both protected and
unprotected online photos of ours.  While several AFR tools have 
provided such measurements ({\em e.g.\/}~\cite{fawkes, foggy}), many others have
not.


% user-deployed AFR tools cannot provide comprehensive protection against unwanted
% FR. {\em Third-party AFR tools} administered by online platforms may provide
% a better long-term solution, despite the resulting loss of user autonomy. Second, researchers proposing new user-centric AFR tools which protect online
% images (e.g. stage $\crc{4}$) must measure and report how
% the presence of unprotected user images in a FR system, alongside
% protected ones, impacts tool performance. Although several AFR tools do
% provide such measurements, e.g. \cite{fawkes, foggy}, many others have
% not.

%  For better or for worse, most people have the same face their whole life~\footnote{Major
% plastic or reconstructive surgery excepted.}. Our faces change as we
% age, but they remain recognizable as uniquely ``us'' to most
% humans. Prior work shows that FR accuracy remains high
%  even with a $10$ year age gap between the reference and test
% images~\cite{ling2009face}. The slow rate at which faces change is a
% major challenge for AFR tools. To be long-term effective, these tools
% must conceal the same piece of static data (a face) from numerous
% adversaries over many years.


% \para{Potential Directions.} {\em Third-party AFR tools} provided by
% online platforms, coupled with enhanced anti-scraping techniques,
% could provide comprehensive protection for users. 



%  Given the online nature of life today, completely eliminating online's
% footprint is a difficult task. However, the burden of protection need
% not rest solely on the  individual.




\noindent\rule{\linewidth}{0.4pt}
 {\bf Challenge 3:  Power asymmetry between FR and AFR}
%Power dynamics favor FR systems} \\
 \noindent\rule{\linewidth}{0.4pt}
% \begin{itemize}
%     \item \cite{oriole} Oriole -- adds cloaked images to the training dataset (i.e. robustness training) to thwart Fawkes. 
%     \item \cite{savior} Data Poisoning Won't Save You -- shows that poisoning methods aren't future-proof and also can't provide a-priori protection. 
%     \item \cite{faceguard} FaceGuard -- removes adversarial perturbations from images to preserve facial recognition accuracy. 
% \end{itemize}

A recent article by Radiya-Dixit and Tramer provides a sharp and
thought-provoking critique of AFR tools~\cite{savior}. They show how the threat model of AFR tools
(especially, but not limited to, those targeting stage $\crc{4}$)
fundamentally favors the FR system \adv~over \pr. Their work argues
that \pr~generally has only a single chance to protect their
image with an AFR tool, while \adv~has numerous opportunities to break
that protection.  That is, once \adv~has access to \pr's protected photo, they can try as many times as they want to break the
protection. \pr~can neither redo their protection on this photo once
\adv~ has it nor predict which techniques \adv~might employ. If
\adv~ever succeeds, either in 1 month or 1 year, they ``win'' and
\pr~loses (since an adult person's face changes very slowly).   Clearly, this asymmetry poses a significant challenge for
AFR development. 

%\para{Key Insights.} 


We note that this asymmetry extends beyond intentional actions by \adv~to
overcome AFR tools. Even passive improvements to FR systems (often triggered
by financial incentives), such as
arrival of 
new training methods or architectures, can overcome AFR protection and
compromise user privacy~\cite{savior}. In 2020, the global FR market
was valued at 3.86 billion US dollars~\cite{global_money}, a huge amount
compared to the 32 academic papers published on AFR tools in the last
ten years. Together, these unfavorable power dynamics and
financial incentives mean that AFR tools face an upward
battle in the fight against unwanted FR. 

\para{Potential Directions.} 
While 
fundamentally the balance rests in favor of FR system developers and
operators, we believe 
legislative efforts and
better platform-level protection (c.f. challenges 2 and 4) may help
address/adjust the power asymmetry between FR and AFR. 


\noindent\rule{\linewidth}{0.4pt}
{\bf Challenge 4: Resisting unregulated, ubiquitous FR \\ deployment}\\
\noindent\rule{\linewidth}{0.4pt}

Today, FR systems are generally unregulated and
easy to deploy.  Practically anyone
 with a powerful laptop and access to an image dataset could create a
 FR system.  This democratization of FR has allowed 3rd party FR systems like Clearview.ai, which rely on unauthorized data
  use~\cite{clearview_explained}, to flourish.  As a result, it is extremely difficult (if not
 impossible) for individuals to know when/where FR systems are
 deployed and what they are capable of. 


% These two factors mean that it is difficult (if not
% impossible) for individuals to know when facial recognition systems
% are deployed and what they are capable of. The lack of regulation has
% led both public and private entities to eagerly adopt FR, as described previously
% (\S\ref{sec:back}). Furthermore, recent technical advances mean that practically anyone
%  with a powerful laptop and access to an image dataset could create a FR system. The democratization of FR has
%  allowed systems like Clearview.ai, which relies on unauthorized data
%  use~\cite{clearview_explained}, to flourish.

This lassiez-faire climate creates significant ambiguity as to when AFR tools can/should be deployed.
For example, around the world, photos taken for official government
purposes ({\em e.g.\/} drivers' license and passport photos) are used as
reference images in government FR systems aiding law enforcement
officers,  border control agents, among others~\cite{perpetual, israel_fr, cbp_facialrec,
  mozur2019one}. This goverment-sponsored FR may be {\em unwanted} but is not (necessarily) {\em unauthorized} under
the status quo, and the legality of using AFR tools to thwart
downstream FR when official driver's license photos are taken is
ambiguous. To augment the confusion, systems like Clearview are used by law
enforcement~\cite{hill_clearview}, further blurring the concept of {\em
  unauthorized} vs {\em unwanted} FR and the appropriate use of AFR tools.

 % For example,
% there are numerous situations in which images may be captured and used
% in FR systems without the possibility of deploying AFR tools. 
%While commercial use of FR has its own
%problems, unregulated FR use by goverment means 
%  . nly a few governments have taken steps to
% curtail FR use through law~\cite{bipa, china_ban_commercial}. However,
% even in these places, law enforcement and other government entites have
%  adopted FR for a variety of uses, perhaps reducing internal governmental
%  pressure to implement more meaningful legislation.

\para{Potential Directions.} Effective FR legislation should focus on
two key points. First, it should determine {\em who is allowed to use FR systems.} This would
clarify when FR systems are or are not unauthorized. A few recent legislative efforts have begun to answer
this question, such as the Illinois Biometric Information Privacy
Act~\cite{bipa}, which sets strict standards for when and how face
data can be used, and China's recent requirement that companies must
ask permission before collecting face
data~\cite{china_ban_commercial}. Second, legislation should determine
{\em when AFR tools can be deployed.} No current
legislation has considered this question, and specific answers to this
question would clarify when individuals can take action against
unwanted FR. As FR and AFR use increases, a clash over this issue seems almost inevitable. 

% Regulation and legal precedent must be established to
% determine if AFR tools can be used against all {\em unwanted} FR or
% only against {\em unauthorized} and {\em unwanted} FR systems.  Legislative efforts
% can augment user- and system-level AFR tools by restricting FR
% use. Specific helpful legislative actions include regulating corporate
% use of facial recognition, providing legal protections for face
% biometric data, and establishing specific guidelines for how and when
% law enforcement agencies can use FR.

% However, general regulation of FR
% technology is elusive. While effective, legislative efforts are
% limited by geopolitical regions, implementation concerns, and delayed
% reaction time. As a result, legislative efforts alone are not
% sufficient to address the privacy concerns of facial recognition in the near future. This leaves a crucial gap which must be filled by AFR tools.

% {\em Solution: Remove task irrelevant information $\crc{1}$.} Face images can include an abundant amount of 
% \emph{task-irrelevant} content that leak unnecessary information. Task-irrelevant content includes content that is
% irrelevant for intended use of the image (\eg bystanders in a selfie) or redundant (\eg video
% stream of a customer taken by a theft detection camera or a traffic violation camera). 
% These task-irrelevant content contains rich data for any facial recongition that can be used to 
% create reference database or as query images. Removing this
% content can significantly reduce the amount of data available to \adv 
% and protect \pr's privacy. Although users could remove this information
% manually in some cases, camera makers or online platforms could do so
% at scale, lowering cost and increasing efficiency.




%\para{Potential Directions.}





==> poison.tex <==
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

\section{Stage $\crc{3}$: Corrupt Extractor Training}
\label{sec:poison}
\shawn{
% Despite the numerous AFR approaches in stage $\crc{1}$, 
It is  challenging, if not impossible, to completely prevent data collection. Therefore, 
many AFR proposals assume that data collection is inevitable and
instead try to corrupt the labelled face data collected by $A$. Such proposals target
two stages: 1) stage $\crc{3}$, where AFR prevents $A$ from training a
successful face feature extractor, and 2) stage $\crc{4}$, where AFR
corrupts the feature database directly. 
}




%\subsection{Threat Model}
\para{$U$'s Goals.} In stage $\crc{3}$, $U$'s goal
is to prevent their photos from being used to train an unauthorized
feature extractor. We assume the data arrived in the training dataset
either through image capture or scraping. We further assume that $U$
attempts to disrupt the training of an {\em unauthorized} facial
recognition system. Table~\ref{tab:consent} presents a non-exhaustive
list of ways in which user photos could be included in a training dataset.

In stage $\crc{4}$, $U$'s goal is disrupt the feature vector creation process. This prevents $A$
from creating an accurate feature vector which can be matched against query images of $U$'s face. As before, $U$ may attempt to disrupt feature vector
creation by posting modified images of themself online or using other
means to disguise their true identity.  

\para{$A$'s Goals.} In stage $\crc{3}$, $A$'s goal is to train a usable feature extractor
from available data. The array of training data available to $A$ is
constrained by their relative power, as illustrated in
Table~\ref{tab:consent}. A low-power adversary may only have access to
limited academic training datasets, while a high-power adversary may
have access to specialized datasets, i.e. government databases or
corporate datasets.

In stage $\crc{4}$, $A$ obtains a feature extractor $\Phi$ and uses
it to create a labeled image database against which
they can run facial recognition searches. This database should contain
feature vectors of the people $A$ wishes to recognize. The
people in the database may be constrained by $A$'s specific
context, \ie if $A$ is a police department, their database should contain criminal suspects.


\subsection{Stage $\crc{3}$: Poison Feature Extractor}

Techniques for poisoning machine learning models are well-known (see
\S\ref{sec:back}). Several recent works have applied data poisoning
methods in the context of facial recognition to mislead
models. Current proposals in this area attempt to {\em make data
  unlearnable}, disrupting extractor training.

Huang \etal~\cite{unlearnable} render training data
``unlearnable'' by a model via specially crafted noise. This noise
misleads the model into thinking the data have already been learned,
thwarting necessary parameter updates. Consequently, the model will not learn anything from the user's
data, protecting their privacy. The unlearnable noise can be
applied to individual examples or an entire class. 

A related proposal from Evtimov \etal~\cite{evtimov2021disrupting}
injects \emph{adversarial shortcuts} into the dataset. Models trained on
this data overfit to the shortcut and fail to learn the meaningful, underlying
semantic features of the data. The model then has a distorted
understanding of the feature space and is useless for generating
feature vectors.

\subsection{Stage $\crc{4}$: Corrupt Reference Database}
\label{sec:corrupt}

%\subsection{Current Stage $\crc{4}$ Proposals} 

As \S\ref{sec:back} discusses, commercial entities often
sell feature extractors to government or private entities. This
entity then creates a labeled reference database containing
feature vector/identity pairs, which will be
used to match incoming query images with their true identity. Several
AFR proposals poison feature vectors added to the reference
database. All proposals are similar but make different assumptions
about how query images are compared to the feature vector database.

\para{Classification-based Matching.} The first two proposals,
Fawkes~\cite{fawkes} and FishyFace~\cite{fishy}, assume that a shallow
classification model is added on top of the feature extactor. The
model is trained to distinguish between elements in the feature vector
database and is used to classify query images.  Fawkes, a
highly publicized~\cite{fawkes_nyt} proposal in this area, poisons the
classification process by ``cloaking'' images, \ie shifting their feature vectors
away from the correct representation by adding imperceptible
perturbations to the input images. Shallow classification models trained on these cloaked
images will learn to associate incorrect feature spaces with the user
identity, producing wrong matches for query images. An earlier
identity-disruption proposal, FishyFace~\cite{fishy}, assumes an SVM is used for
end-classification on a feature extractor and adds adversarial
perturbations to images which disrupt SVM classification.

\para{KNN Matching.} The other proposals, LowKey~\cite{lowkey} and
FoggySight~\cite{foggy}, assume a k-nearest neighbors approach to query/database matching.  LowKey~\cite{lowkey} adds digital adversarial perturbations to
change the feature representation of $U$'s images (similar to Fawkes). These perturbed images create an
incorrect feature vector for $U$ and thus prevent FR from successful
matching. FoggySight~\cite{foggy} instead focuses on a
community-driven approach, where users modify their
images to protect others. These collective modifications flood the top-K matching set for a specific
user with incorrect feature vectors, drowning out the correct feature
vector and preventing query image matching. 

% STAGE 6 threat model
% \subsection{Threat Model ($U$ vs. $\ag$)}

% \para{$U$'s Goals.} 

% \para{$\ag$'s Goals.} 
